Multimodal Abstractive Summarization for How2 Videos

In this paper, we study abstractive summarization for open-domain videos. Unlike the traditional text news summarization, the goal is less to "compress" text information but rather to provide a fluent textual summary of information that has been collected and fused from different source modalities, in our case video and audio transcripts (or text). We show how a multi-source sequence-to-sequence model with hierarchical attention can integrate information from different modalities into a coherent output, compare various models trained with different modalities and present pilot experiments on the How2 corpus of instructional videos. We also propose a new evaluation metric (Content F1) for abstractive summarization task that measures semantic adequacy rather than fluency of the summaries, which is covered by metrics like ROUGE and BLEU.

==> final/5related_work.tex <==
\begin{figure*}[t]
  \centering
  \includegraphics[ trim={0 5cm 0 0}, clip, width=\linewidth]{figures/copy_of_how2example.pdf}
  \caption{How2 dataset example with different modalities. ``Cuban breakfast'' and ``free cooking video'' is not mentioned in the transcript, and has to be derived from other sources.}
  \label{fig:how2data}
\end{figure*}

Summarization is a challenging task that involves understanding the important information of a document and generating a shorter summary by preserving and aggregating the important information in the document. Summarization has been studied for both textual documents (automatic text summarization) and visual documents such as images and videos (video summarization). 
Automatic text summarization is a widely studied topic in natural language processing \cite{luhn1958automatic,kupiec1995trainable,mani1999advances}, given a text document task is to generate a textual summary for applications that can assist users understand large documents.
Most of the work on text summarization has focused on single-document 
summarization for domains such as news \cite{rush2015neural,cnndm_nallapathi,see2017get,narayan2018ranking} and a few on multi-document summarization \cite{goldstein2000multi,lin2002single,woodsend2012multiple,cao2015ranking,YasunagaZMPSR17}.

Video summarization is the task of producing the compact version of the video (visual summary) by encapsulating the most informative parts. It involves identifying series of key frames that depict the essential events in the video \cite{money2008video,lu2013story,gygli2014creating,song2015tvsum,sah2017semantic}. Our task of multimodal summarization is the task of summarizing a video document with a text summary that summarizes the content of the video i.e., generating a textual summary for video content. A closely related task to ours is video title generation where the task is to describe the most salient events in the video in a compact title that can capture users attention \cite{zeng2016generation}. Other related work include video captioning and description generation which focus on activities or story of the video and generate descriptions at various levels of granularity from single sentence to multiple sentences, multimodal summarization of images and text \cite{DaXuDoCVPR2013,RegneriRWTSP13,RohrbachRQFPS14,ZhouXC18,gella2018dataset,zhu2018msmo}.

Multimodal summarization is a more recent challenge with yet no benchmarking datasets yet. \citet{li2017multi}
collected a multimodal corpus of 500 English news videos and 
articles paired with manually annotated summaries. The dataset is small-scale and has news articles with audio, video, and text summaries, but there is no human annotated audio-transcripts. In our summarization task, we focus on describing the intent of the video and stating the exclusive and unique features of the video, irrespective of modality. This summary can thus be thought of like a textual ``teaser'' or title for the video.

